FoReCo: a forecast-based recovery mechanism for real-time remote control of robotic manipulators

Wireless communications represent a game changer for future manufacturing plants, enabling flexible production chains as machinery and other components are not restricted to a location by the rigid wired connections on the factory floor. However, the presence of electromagnetic interference in the wireless spectrum may result in packet loss and delay, making it a challenging environment to meet the extreme reliability requirements of industrial applications. In such conditions, achieving real-time remote control, either from the Edge or Cloud, becomes complex. In this paper, we investigate a forecast-based recovery mechanism for real-time remote control of robotic manipulators (FoReCo) that uses Machine Learning (ML) to infer lost commands caused by interference in the wireless channel. FoReCo is evaluated through both simulation and experimentation in interference prone IEEE 802.11 wireless links, and using a commercial research robot that performs pick-and-place tasks. Results show that in case of interference, FoReCo trajectory error is decreased by x18 and x2 times in simulation and experimentation, and that FoReCo is sufficiently lightweight to be deployed in the hardware of already used in existing solutions.

==> AIC_dif.tex <==
\subsection{Notes on difference order}
{\color{red} Figure~\ref{fig:aic-impact} shows that
there is very little improvement in our model.
Using Carlos data $AIC_{0}-AIC_{19}=49$, hence
the likelihood is only $<0.0001$ times better than
not using past information}

VAR estimates the six joints position $y\in\mathbb{R}^6$
using the $l$ previous lags, i.e., the previous joints
positions; and a matrix of parameters $A_i\in\mathbb{R}^{6\times6}$
for each $i$-th lag:
\begin{equation}
    y_t = \sum_{i=1}^l A_i\cdot y_{t-i} + e_t
    \label{eq:var}
\end{equation}
with $e_t$ denoting the prediction error of VAR at time $t$.

We measure the improvements of the VAR accuracy using the
AIC metric $AIC=2\cdot p- \log \hat{L}$. Where $p$ is the
number of estimated parameters in the model, and $\hat{L}$
is its likelihood. In the case of VAR there are
$p=6^2\cdot l$ parameters to be estimated, that is, the
$l$ parameter matrices $A_i$. Thus, the likelihood
improvement of
a VAR model with lag order $l$, and a VAR model with
lag order $l+1$ is expressed as:
\begin{equation}
    \frac{\hat{L}_{l+1}}{\hat{L}_l} = e^{\frac{AIC_l-AIC_{l+1}}{2}+6^2}
    \label{eq:lag-improve}
\end{equation}
Figure~\ref{fig:aic-impact} shows how
the $\tfrac{\hat{L}_{l+1}}{\hat{L}_l}$
ratio improves with the AIC difference
of models differing on only one lag order.
Our experiments showed two notorious
improvements in the AICs, in particular,
in $AIC_0-AIC_1=43.45$,
$AIC_4-AIC_5=4.8$. According to
Figure~\ref{fig:aic-impact}, this means
that the likelihood of using $l=1$
is $10^{25}$ times better than $l=0$,
and the likelihood of using $l=5$ is
$10^{17}$ times better than using
only $l=4$ lags.
With $l>5$, no
matter how much the lag order is increased,
the AIC metric reamains always above
$79$, as it penalizes the overfitting
derived of the increasing number of
parameters.

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{img/aic-var-diff-order.eps}
    \caption{Impact of AIC difference in VAR models likelihood}
    \label{fig:aic-impact}
\end{figure}

